General Holder Smooth Convergence Rates Follow From Specialized Rates Assuming Growth Bounds

Often in the analysis of first-order methods for both smooth and nonsmooth optimization, assuming the existence of a growth/error bound or KL condition facilitates much stronger convergence analysis. Hence separate analysis is typically needed for the general case and for the growth bounded cases. We give meta-theorems for deriving general convergence rates from those assuming a growth lower bound. Applying this simple but conceptually powerful tool to the proximal point, subgradient, bundle, dual averaging, gradient descent, Frank-Wolfe, and universal accelerated methods immediately recovers their known convergence rates for general convex optimization problems from their specialized rates. New convergence results follow for bundle methods, dual averaging, and Frank-Wolfe. Our results can lift any rate based on H\"older continuous gradients and H\"older growth bounds. Moreover, our theory provides simple proofs of optimal convergence lower bounds under H\"older growth from textbook examples without growth bounds.

==> conclusion.tex <==
\section{Conclusion}
For a wide class of first-order methods, we have shown that conducting separate analysis under different growth conditions (or lack thereof) is unnecessary. Given a convergence rate assuming a growth bound, general convergence guarantees and guarantees relying on weaker growth bounds follow from our rate lifting theorems. Applying restarting schemes like~\cite{RenegarGrimmer2021} gives the converse, allowing improved growth bounded convergence rates to be derived from general rates. As a result, with only minor algorithmic modifications, it suffices to analyze the first-order method in any one of these settings. Then meta arguments can be made to derive the convergence rates in all the other cases.

The analysis machinery developed herein applies to the wide family of H\"older-smooth optimization problems and allows for backward-steps like those used by the proximal point method. One interesting future direction based on these results would be the analysis of composite optimization problems, minimizing the sum of two functions $f+g$. Such structured objectives are commonly addressed using proximal gradient methods or splitting algorithms. These methods are known to speed up under the same H\"older growth conditions considered here and so generalizing our rate lifting theorems may be possible.
